Representation Integrity in Temporal Graph Learning Methods

Real-world systems ranging from airline routes to cryptocurrency transfers are naturally modelled as dynamic graphs whose topology changes over time. Conventional benchmarks judge dynamic-graph learners by a handful of task-specific scores, yet seldom ask whether the embeddings themselves remain a truthful, interpretable reflection of the evolving network. We formalize this requirement as representation integrity and derive a family of indexes that measure how closely embedding changes follow graph changes. Three synthetic scenarios, Gradual Merge, Abrupt Move, and Periodic Re-wiring, are used to screen forty-two candidate indexes. Based on which we recommend one index that passes all of our theoretical and empirical tests. In particular, this validated metric consistently ranks the provably stable UASE and IPP models highest. We then use this index to do a comparative study on representation integrity of common dynamic graph learning models. This study exposes the scenario-specific strengths of neural methods, and shows a strong positive rank correlation with one-step link-prediction AUC. The proposed integrity framework, therefore, offers a task-agnostic and interpretable evaluation tool for dynamic-graph representation quality, providing more explicit guidance for model selection and future architecture design.

==> Chapters/abstract.tex <==
Real-world systems ranging from airline routes to cryptocurrency transfers
are naturally modeled as \emph{dynamic graphs} whose topology changes over
time.  Conventional benchmarks judge dynamic--graph learners by a handful of
task-specific scores, yet seldom ask whether the embeddings themselves
remain a truthful, interpretable reflection of the evolving network.
We formalize this requirement as \textbf{representation integrity} and derive a family of property-based indexes that measure how closely embedding
changes follow graph changes.  Three synthetic streams---\emph{Gradual
Merge}, \emph{Abrupt Move}, and \emph{Periodic Re--wiring}---are used to screen forty--two candidate indexes; we choose one index that passes every theoretical and
empirical test.  When applied
to eight representative models, this validated metric (i) consistently ranks
the provably stable UASE and IPP embeddings highest, (ii) exposes the
scenario--specific strengths of neural methods (DynAE under smooth drift,
DynRNN under sudden jumps), and (iii) shows a positive rank correlation
with one--step link--prediction AUC (\(\rho\!\approx\!0.60\)).
The proposed integrity framework, therefore, offers a task-agnostic
and interpretable evaluation tool for dynamic-graph representation quality, providing more explicit guidance for model selection and future architecture design.
